Efficiently Quantifying Individual Agent Importance in Cooperative MARL

Measuring the contribution of individual agents is challenging in cooperative multi-agent reinforcement learning (MARL). In cooperative MARL, team performance is typically inferred from a single shared global reward. Arguably, among the best current approaches to effectively measure individual agent contributions is to use Shapley values. However, calculating these values is expensive as the computational complexity grows exponentially with respect to the number of agents. In this paper, we adapt difference rewards into an efficient method for quantifying the contribution of individual agents, referred to as Agent Importance, offering a linear computational complexity relative to the number of agents. We show empirically that the computed values are strongly correlated with the true Shapley values, as well as the true underlying individual agent rewards, used as the ground truth in environments where these are available. We demonstrate how Agent Importance can be used to help study MARL systems by diagnosing algorithmic failures discovered in prior MARL benchmarking work. Our analysis illustrates Agent Importance as a valuable explainability component for future MARL benchmarks.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/9-checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{relatedwork}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> sections/previous_work/0-abstract.tex <==
\begin{abstract}

% very very rought first draft. please feel free to edit without even making comments. 

Cooperative multi-agent reinforcement learning (MARL) has made impressive strides in solving distributed decision-making problems. However, as multi-agent systems become more complex, understanding their behaviour becomes increasingly challenging. In this paper, we compile a suite of MARL diagnostics: metrics and interpretability tools designed to identify critical algorithmic issues and help uncover unintuitive behaviour between agents. Our analysis of well-known algorithms validates the effectiveness and importance of having interpretability diagnostics. Notably, we provide insights into instances of unexpected algorithmic performance. In RWARE we are able to show that the poor performance of Q-Learning methods is not only due to sparsity but also due to relative action importance adversely affecting random sampling and in LBF that Multi-Agent Proximal Policy Optimization (MAPPO) can become trapped in local minima due to early over-training. We also show that in purely cooperative settings, difference rewards can be used to accurately calculate per agent importance values that are identical to Shapley Values with lower computational costs. Finally, the diagnostics suite for this analysis is open-sourced as a repository for seamless integration into various frameworks, assisting in automating the analysis and evaluation of algorithms in future work.

\begin{comment}
such as when Independent Q-Learning (IQL) outperforms Value-Decomposition Networks (VDN) and QMIX on cooperative tasks, and when Multi-Agent Proximal Policy Optimization (MAPPO) is outperformed by Multi-Agent Advantage Actor-Critic (MAA2C). The diagnostics suite for this analysis is open-sourced as a library for seamless integration into various frameworks, assisting in automating the analysis and evaluation of algorithms in future work.\\


The mostly commonly tracked metric in cooperative multi-agent reinforcement learning research is the team reward over time which makes sense as a way to quantify whether agents are learning optimal policies to solve the task at hand. We argue that the reward might hide underlying information about the true behaviours of these agents and suggest a suite of metrics that can be used to uncover the nature of agent policies without having to resort to rendering an environment. 
\end{comment}

\end{abstract}

==> sections/previous_work/1-introduction.tex <==
\section{Introduction}

\begin{comment}
In recent years, multi-agent reinforcement learning (MARL) has grown immensely as a field \cite{mahajan2019maven} \cite{rashid2018qmix} \cite{SMAC} \cite{wang2020roma}.
\end{comment}

In recent years, multi-agent reinforcement learning (MARL) has achieved significant progress, with agents able to outperform human players and develop complex coordinated strategies in difficult games such as \textit{Starcraft} \citep{SMAC, Vinyals2019GrandmasterLI} and \textit{Hanabi} \citep{foerester2019bad, Hanabi, hu2021simplified,  wei2021mad}. Furthermore, MARL has also shown promising results in solving real-world problems such as network resource allocation and sharing, network routing, and traffic signal controls \citep{DynamicPowerAllocation, InternetofControllableThings, IoTNetworksWithEdgeComputing, TrajectoryDesignandPowerAllocation, brittain2019autonomous, IntelligentTrafficControl, AirTrafficManagement}.

\begin{comment}
    Despite the tremendous advances in this field, various challenges keep posing roadblocks to further growth. One highly highlighted issue is the difficulty of replicating algorithm components accurately \cite{hu2022rethinking}\cite{engstrom2020implementation} \cite{henderson2019deep}. To address this problem, recent efforts have focused on developing fair comparison techniques using statistical measurements of performance \cite{gorsane2022standardised} \cite{jordan2020evaluating} \cite{agarwal2022deep}. These works also suggest methods that can be used to make inter-paper results easier to compare which aids in accurately assessing the growing body of algorithms in MARL. However, these techniques are primarily focused on determining the final performance of the algorithm, and may not effectively capture the strengths and weaknesses of the algorithm or interpret the emergent behavior within the system. 
\end{comment}

\begin{comment}
    The field of MARL has experienced significant growth and complexity, making it increasingly challenging to pinpoint the exact causes of algorithmic performance on a given benchmark (Henderson et al., 2018; Engstrom et al., 2020; Hu et al., 2022a). Additionally, the rapid development of MARL algorithms has led to increased complexity in published works (Sunehag et al., 2017a; Rashid et al., 2018a; Peng et al., 2021), leading to a growing concern regarding statistical performance measurements in reinforcement learning. Researchers have proposed new methods for comparing results across studies, which have aided in accurately assessing the expanding body of algorithms (Gorsane et al., 2022; Agarwal et al., 2022; Jordan et al., 2020).
\end{comment}

As the field of MARL has grown in scope and complexity, pinpointing the exact cause of algorithmic performance on a given benchmark has become increasingly challenging \citep{henderson2019deep, engstrom2020implementation, hu2022rethinking}. Reinforcement learning, in general, has faced increasing scrutiny regarding statistical performance measurements \citep{gorsane2022standardised, agarwal2022deep, jordan2020evaluating}. These works propose methods to facilitate inter-paper result comparisons, which aids in accurately assessing the expanding body of algorithms. However, the rapid development of MARL algorithms has has also led to increased complexity in  published works \citep{VDN, QMIX, FACMAC}. %move this up

%Add more citations to this
\begin{comment}
    With the increase in the complexity of recent works \cite{VDN} \cite{QMIX} \cite{FACMAC}, there is a need for more research into understanding the underlying mechanisms and characteristics of Marl algorithms to enable their optimal use in various applications. However, it is equally essential to uncover any underlying failures that may impact the algorithm's performance. Despite achieving high team returns, an algorithm may still suffer from issues such as \textit{reward hacking}, \textit{coordination failures}, \textit{overfitting}, \textit{limited scalability}, and \textit{a lack of transparency}. Reward hacking occurs when agents manipulate the reward function, While coordination failures arise from inefficient communication. Overfitting and limited scalability make the algorithm infeasible for larger problems. Working with black-box systems may also result in a lack of transparency, which hinders progress and improvement. Such issues could lead to unstable performance when replicating the algorithm or changing the training environment.

    In this context, many efforts have been made in various directions to tackle the cited challenges... (TODO: add related work shapley value, melting pot, bsuite...)
\end{comment}

\begin{comment}
    Despite the progress made in evaluating MARL algorithm performance, the explanatory side of these algorithms has not yet been fully explored. Standard methods for evaluating MARL in the cooperative setting rely on measuring empirical returns or statistics derived from them (Gorsane et al., 2022). Although more robust solutions have been developed (Agarwal et al., 2022), these methods are insufficient to explain the behavior of RL algorithms. In the single-agent setting, the Behaviour Suite for Reinforcement Learning (BSuite) framework has become a popular choice for benchmarking RL algorithms due to its comprehensive diagnostic tools for analyzing agent behavior (Citation). BSuite offers a suite of experiments to evaluate various aspects of agent behavior, including generalization, exploration, and credit assignments. In addition to BSuite, ShinRL (Kitamura and Yonetani, 2021) is a powerful analysis tool that generates empirical evidence for the theoretical properties of deep RL algorithms. ShinRL includes state and action space visualizations, reward distributions, and other diagnostic tools that provide researchers with insights into the behavior of agents and potential issues with RL algorithms. In the multi-agent settings, there are also some efforts in coming up with metrics to diagnose the performance of the agents (citation of agent diversity paper, smarts, melting pot, shapley value ones). Despite these efforts, there is still a need to gather these metrics in a unified toolbox library. Furthermore, some of these metrics are specific to certain environments and may not be applicable in other settings, and their implementation can be complex. Therefore, there is a need to develop environment-free and less complex metrics that can be applied across various settings and incorporated into a comprehensive toolkit for evaluating multi-agent reinforcement learning algorithms.
\end{comment}
Standard methods for evaluation of MARL in the cooperative setting rely on measuring the empirical returns or statistics derived from them \citep{gorsane2022standardised}. Although these methods have come under scrutiny and more robust solutions have been developed \citep{agarwal2022deep}, they are insufficient to explain the RL algorithm behavior. In the single-agent setting, frameworks have been developed to better explain how methods work \citep{ShinRL}. In MARL, while some works explore metrics like agent diversity, they are not consolidated into a unified framework, necessitating additional efforts from individual researchers.

%More citation
\begin{comment}
    In this paper, we argue the necessity of advanced metrics to diagnose the algorithm performance rather than relying purely on traditional evaluation metrics such as team return... 
    (TODO: extend this section with the proposal above + annotate the contribution that we've made by insisting on the automated library that can easily be integrated into any framework and that it won't affect the training time as we make it robust and not a time consumer...)
\end{comment}
\begin{comment}
    In this paper, we argue that to advance the field of RL and expand its current state of the art to real-life applications, it is imperative to consider not only the empirical performance of the algorithm but also understand the behavior of the agents and the system dynamics. Moreover, gaining insight into the strengths and limitations of the algorithm will enable us to optimize it more effectively. Our work involves adapting several behavior analysis methods to the multi-agent reinforcement learning (MARL) setting. Through redoing the Level-Based Foraging (LBF) and Multi-Robot Warehouse (RWARE) environments experiments from the cooperative marl benchmark paper (citation), we demonstrated how these methods can provide additional insights during and after algorithmic training, without introducing any significant overhead or affecting the training process. We also show how behavior explanation can help diagnose and detect common MARL algorithm failure cases, which are typically challenging to identify. Furthermore, we compiled the metrics into an open-source library available at [some link] for easy integration and made all the experiment raw data results publicly available for reproducibility and analysis purposes.
\end{comment}
In this paper, we argue that it is necessary to not solely rely on empirical performance for evaluating MARL methods; instead, we should also track metrics providing direct insights into agent behavior. To accomplish this, we adapt multiple implementation agnostic behavior analysis methods to the MARL setting, show how these can be used to detect and analyse common MARL failure cases and present a novel method for agent importance calculation which has linear scaling with coalition size. Finally, we compile these metrics into an open-source repository available at [some link] for easy integration.

==> sections/previous_work/2-metrics-draft.tex <==
\section{Metrics}
In order to evaluate agent behavior we make use of several metrics. This section presents a compilation of behavior explanation metrics to diagnose the learned policies of multi-agent reinforcement learning (MARL) algorithms. We provide background on metrics from existing works, their practical adaptation to the MARL setting and to the best of our knowledge, are the first to use difference rewards to explain \textit{agent importance}.

\begin{comment}
    This section presents a compilation of sophisticated metrics utilized for troubleshooting algorithm performance to guarantee its accuracy. We emphasize the essential elements that require assessment, including the metrics adopted from previous studies, and conclude each element by introducing the novel metrics that our library has incorporated.
\end{comment}


\subsection{Related Works}

\textbf{Shapley Values:} The Shapley Values are a famous method used to solve the issue of payoff distribution for the grand coalition \citep{shapley1953}. Meaning it it used to determine the contribution of each member of the coalition towards completion of a task. Given a cooperative game $\Gamma = (\mathcal{N},v)$ for any $\mathcal{C} \subseteq \mathcal{N}/\{i\} $ let $\phi_{i}(\mathcal{C}) = v(\mathcal{C} \cup \{i\}) - v(\mathcal{C})$ be a marginal contribution, the Shapley Value of each agent $i$ can be written as:
\begin{equation}
Sh_{i}(\Gamma) = \sum_{\mathcal{C} \subseteq \mathcal{N}/\{i\}} \frac{|\mathcal{C}|!(|\mathcal{N}| - |\mathcal{C}|-1)!}{|\mathcal{N}|!} \cdot \phi_{i}(\mathcal{C})
\end{equation}

%Word this better
Where $\mathcal{N}$ is a set of agents, $v$ is the value function used to measure the profits earned by the coalition which maps from a coalition $\mathcal{C} \subseteq \mathcal{N}$. The set of agents $\mathcal{N}$ is also referred to as the grand coalition and contains all agents.

Calculating Shapley values presents two issues, it requires the computation of $2^{n-1}$ possible coalitions of a potential $n(2^{n-1})$  coalitions which is computationally expensive and ideally is used in a simulator where where agents can be removed from the coalition and the value of the same states to be evaluated with each coalition.

To make these calculations reasonable, we can instead compute the contributions based on a subset of the coalitions instead of all possible coalitions. We can do this by reformulating the Shapley value calculation as a Monte-Carlo estimate \citep{monte1949}...%Add derivation from paper on notion

This reinterpretation of the Shapley values can be calculated as:
\begin{equation}
\hat{\phi}^{RL}_{i}(r) = \frac{1}{M} \sum^{M}_{m=1}(r^{m}_{+i} - r^{m}_{-i}) \approx \phi_{i}(r)
\end{equation}
Where $\hat{\phi}^{RL}_{i}(r)$ is the shapley value for agent $i$ given joint reward $r$, $M$ is the total number of coalitions sampled, $r^{m}_{+i}$ is the return for coalition $m$ out of all possible coalitions $M$ with agent $i$ and $r^{m}_{-i}$ is the return for coalition $m$ out of all possible coalitions $M$ without agent $i$

%KL divergence
\textbf{Kullback–Leibler (KL) divergence:} An intuitive solution, proposed by prior work to determine the difference between the policies of multiple agents is to measure the KL divergence between the agent policies at each timestep of evaluation however, the KL divergence when used as the sole agent explanation method can give misleading feedback regarding the agent policies. Despite the intuition that actions taken at the same timestep can indicate different roles \citep{wang2020rode} this is often not the case. Over the course of a trajectory, agents may have very similar policies overall but individual steps with high divergence due to their differing observation spaces \citep{hu2022policy}. As an example, in a game of football, four players have the role of a defender but, given their observations of the game state and their own positions they would have to react differently to fulfil their assigned roles \citep{kurach2020google}. 
\subsection{Actions diversity}
During the training of MARL systems, the agents within the coalition will naturally move into more defined roles over time. This role is not inherently defined by the type of agent but rather by the trajectory the agent will follow over the course of an episode \citep{wang2020roma,phan2021vast}. Methods like role-oriented MARL (ROMA) make use of deep learning methods like encoders in order to learn an embedding space to improve the learning of MARL algorithms. This provides a built-in method to track role-diversity during training. However, this type of role-oriented framework is not used across all MARL methods and we explore implementation-agnostic methods that can be applied independently to network architecture.

\begin{comment}
    To assess the diversity of agents' actions, one common approach is to calculate the KL divergence between their policies at each timestep of evaluation. However, this method may not provide an accurate representation of diversity since policies can vary significantly based on observations, and agents may have similar policies overall but differing KL divergence values in individual steps due to observation differences (Hu et al., 2022b). As an example, in a game of football, four players have the role of a defender but, given their observations of the game state and their own positions they would have to react differently to fulfill their assigned roles (Kurach et al., 2020).\\ 

    An alternative solution was by defining the action-based role ... (from line 72->81 looks good)
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Task Switching}
\begin{comment}
Based on prior studies, we have established a two-level approach for measuring diversity in task switching. The first level focuses on \textbf{agent action diversity}, which involves tracking the frequency of different actions taken by each agent during evaluation. This information can be used to identify any agents that consistently use the same action or the noop action, indicating laziness, and to assess agent exploration of different actions.

The second level of diversity measurement involves assessing \textbf{agent diversity} by calculating the kl divergence between the action distribution of different agents. By comparing the actions taken by various agents, we can determine whether agents have similar behaviors or different roles. This method enables us to gain insight into the extent of diversity among agents, which can be useful for optimizing task allocation and resource management.
\end{comment}

\begin{comment}
    Task switching is an essential metric for monitoring action usage in multi-agent reinforcement learning (MARL), which allows a thorough examination of the agent's exploration-exploitation balance within its environment, analysis of the agent's learning dynamics, and assessment of diverse learning algorithms and strategies' effectiveness. This metric quantifies the frequency at which an agent selects specific actions..\\

    To track the task switching,  we monitor the usage of each agent action at every timestep $t$ during the evaluation phase of the agent in the training process. By analyzing the recording frequencies, we can compute the likelihood of each action being selected, which we achieve by passing them through a soft-max distribution.  Mathematically it can be described as ...
\end{comment}
\textbf{Task Switching:} By implementing a practical task-switching metric, it becomes possible to quantify the frequency at which an agent selects specific actions during the evaluation phase. This, in turn, enables a thorough examination of the agent's exploration-exploitation balance within its environment, as well as an analysis of the agent's learning dynamics and an assessment of the algorithmic strategy diversity and effectiveness. 

This can be implemented by tracking the usage of each agent action at each timestep $t$ during the evaluation phase of agent training. From the recorded frequencies, we can compute the likelihood of each action being selected by passing the counter through a soft-max distribution to generate a likelihood estimation for each action. Mathematically it can be described as:

\begin{equation}
\mathcal{T}_T = \sigma( \sum^{T}_{t=0} \Vec{a}^{i}_{t})
\end{equation}

Where $\sigma$ is a softmax function used to convert the action counts to a probability distribution, $\Vec{a}^{i}_{t}$ is a one-hot encoded vector of the action chosen by agent $i$ at timestep $t$ and $\mathcal{T}_T$ is a matrix containing the cumulative likelihood of each possible action up until the terminal timestep $T$ for each timestep in the environment $t$.

\begin{comment}
TODO: add equation for kl_div on the probs or just mention it
Monitoring action usage can provide valuable information about the agent learning process in MARL and aid in evaluating the effectiveness of various learning algorithms and strategies. The practical implementation of the task-switching method allows us to measure the frequency an agent takes a specific action during an evaluation phase, allowing us to evaluate the agent's learning to observe how well the agent is exploring-exploiting the environment and to examine the dynamics of the agent's learning.

--------------------------------------------------------------
**Deductions**:

*Learning Dynamics: Tracking action usage provides an indication of how the agent learns. By observing the evolution of action usage over time, we can examine the dynamics of the agent's learning and see whether or not the agent is learning a good policy, so some increase in the usage of actions that lead to higher rewards can be expected.
E.g If an agent's use of actions that result in higher rewards increases, it may imply that the agent is learning an optimal strategy. If, on the other hand, an agent reduces its use of actions that result in lower rewards, it may indicate that the agent is learning to avoid suboptimal behavior.

*Exploration-Exploitation: With the task-switching method we can ensure that the agent explores all possible actions in the environment after each slot of the training phase. This exploration allows the agent to find better policies that result in higher rewards. However, if the agent only explores and never exploits, it may never learn to maximize its rewards.
E.g If an agent consistently chooses the same action, it may be a sign that it's not sufficiently exploring the environment and, therefore, not learning an optimal policy. On the other hand, if an agent explores a wide range of behaviors, it may mean that it is not fully exploiting the best actions and, therefore, not maximizing its rewards.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contribution analysis}

The ability to directly monitor the contributions of individual agents in a MARL system is critical due to the popularity of value-decomposition algorithms for solving cooperative games. Popular algorithms like VDN and QMIX rely on improving multi-agent credit assignment to generate better reward signals. Analysis of these credit assignment schemes can lead to the development of better decomposition methods. However, as these methods are typically trained in an end-to-end manner it is difficult to apply neural network explainability methods to them and built-in explainability is limited to a few explicitly designed algorithms \citep{wang2020shapley, yang2020qatten, yang2020q}. Instead, we propose the use of difference rewards to calculate model agnostic representations of agent importance.

\begin{comment}
Understanding each agent's input is critical since it can provide insight into how the agents are learning and behaving in the environment. This knowledge can be used to create more effective learning algorithms. It enables us to find areas for improvement, create better strategies, and encourage collaboration among agents (for example we can mention the algorithms that used the Shapley value to increase performance).

Some ideas why we should consider this contribution/Shapley value:

- it allows us to improve and evaluate the efficiency of the system: By evaluating the performance of each agent, we can evaluate the overall efficiency of the system and identify which agents are performing well (learning an optimal policy) and which ones may be hindering the performance of the group, and we can use this information to make improvements to the system (for example we can adjust the reward structure or modify the behavior of specific agents/ adjust the agents architecture)

-  it helps to understand the behavior of agents: By analyzing the contribution of each agent, we can better understand how agents interact with each other and how they influence their behavior. This information can be used to develop better strategies to achieve the desired outcome and to identify which agents work well together and which do not, and we can take steps to encourage cooperation between agents (reward shaping: adding a positive reward or a penalty for a specific behavior/ distribute the team reward based each contribution).

\end{comment}

%\subsubsection{Agents importance}

\textbf{Agents importance:} Rather than calculate the expensive Shapley Value of each agent at each timestep, we instead make use of online difference rewards to determine per agent contributions. To overcome the lack of resettable simulators in MARL, we instead create $n$ copies of the training environment where $n$ is the number of agents in the coalition at timestep $t$. We are then able to calculate the difference reward of each agent with respect to the reward of the grand coalition. Mathematically this can be shown as:
\begin{equation}
\hat{\phi}^{RL}_{n}(r) = r_{m} - r_{-n} \approx \phi_{i}(r)
\end{equation}

Where $\hat{\phi}^{RL}_{n}(r)$ is the agent importance for agent $n$ given the group reward of the grand coalition $r_{m}$ and $r_{-n}$ is a copy of the environment where the effect of agent $n$ is minimised. In practice this takes the form of a no-op action. These difference rewards scale linearly in computational complexity with respect to the number of agents in the coalition rather than exponentially like the Shapley Value. %We also find that, in practice, these difference rewards are identical to the true Shapley Value when applied to purely cooperative settings.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training Stability}
\begin{comment}
Understanding the dynamic of a multi-agent reinforcement learning (MARL) system during the learning process is essential for effective and efficient learning. Diagnosing the dynamic of the system can help identify learning instability, slow convergence, and implementation bugs or hyperparameter issues. By being aware of the system's dynamic, we can adjust the learning algorithm or reward function to improve learning and design more robust and effective MARL systems. While our implementation of common methods for measuring training stability may not be considered novel, it is crucial to have them in order to ensure that the learning process is stable and effective.
\end{comment}
%\subsubsection{Agent update divergence}
\textbf{Agent update divergence:} We measure the per step KL divergence of each agent to measure how the policy changes over time. A high KL divergence over time is usually indicative of a stochastic policy and can be thought of as a measurement of agent stability or if the agent policy has converged to an optimal parameterisation. KL Divergence can also be measured on a per agent basis and compared. If individual agents have high KL divergence and other do not, it can indicate a tendency for the MARL policy to overweight certain agents in the coalition and learn unbalanced policies.

%\subsubsection{Team and individual entropy}

\textbf{Team and individual entropy:} It was shown by \cite{abdallah2009global} that using only the global returns as a metric may hide underlying instability in agent policies. They suggest using the agent policy entropy as a proxy for measuring the stability with which an agent $i$ has converged to a certain behaviour. This can be computed as for each agent as 

\begin{equation}
H_i(\pi( \cdot | o^i_t)) = - \sum_{a^i \in A^i} \pi(a^i|o^i_t) \log \pi(a^i|o^i_t))    
\end{equation}

Where $i$ is the id of an individual agent in the coallition, $o$ is an individual agent observation, $a^i$ is the action of agent $i$ at timestep $t$, $\pi$ is the policy of agent $i$ and $H_i$ the entropy of agent $i$. This is extended to the full team by computing the mean team entropy as 

\begin{equation}
%H(\pi( \cdot | o_i, \dots, o_n)) = \mathbb{E}[H_i]    
H(\pi( \cdot | o_i, \dots, o_n)) = \frac{1}{n}\sum^n_{i=0} H_i  
\end{equation}
Where $n$ is the total number of agents in the coalition.


==> sections/previous_work/2-metrics.tex <==
\section{Metrics}
In order to evaluate agent behavior for both offline and online evaluation, we make use of several metrics. This section presents a compilation of behavior explanation metrics to diagnose the learned policies of multi-agent reinforcement learning (MARL) algorithms. We provide background on metrics from existing works and their practical adaptation to the MARL setting.

\begin{comment}
    This section presents a compilation of sophisticated metrics utilized for troubleshooting algorithm performance to guarantee its accuracy. We emphasize the essential elements that require assessment, including the metrics adopted from previous studies, and conclude each element by introducing the novel metrics that our library has incorporated.
\end{comment}

\subsection{Related Works}

\subsection{Actions diversity}
During the training of MARL systems, the agents within the coalition will naturally move into more defined roles over time. This role is not inherently defined by the type of agent but rather by the trajectory the agent will follow over the course of an episode \citep{wang2020roma,phan2021vast}. Methods like role-oriented MARL (ROMA) make use of deep learning methods like encoders in order to learn an embedding space to improve the learning of MARL algorithms. This provides a built-in method to track role-diversity during training. However, this type of role-oriented framework is not used across all MARL methods and we explore implementation-agnostic methods that can be applied independently to network architecture.
\subsubsection{Existing work}
\begin{comment}
    To assess the diversity of agents' actions, one common approach is to calculate the KL divergence between their policies at each timestep of evaluation. However, this method may not provide an accurate representation of diversity since policies can vary significantly based on observations, and agents may have similar policies overall but differing KL divergence values in individual steps due to observation differences (Hu et al., 2022b). As an example, in a game of football, four players have the role of a defender but, given their observations of the game state and their own positions they would have to react differently to fulfill their assigned roles (Kurach et al., 2020).\\ 

    An alternative solution was by defining the action-based role ... (from line 72->81 looks good)
\end{comment}

An intuitive solution, proposed by prior work to determine the difference between the policies of multiple agents is to measure the KL divergence between the agent policies at each timestep of evaluation however, the KL divergence in isolation can give misleading feedback regarding the agent polcies. Despite the intuition that actions taken at the same timestep can indicate different roles \citep{wang2020rode} this is often not the case. Over the course of a trajectory, agents may have very similar policies overall but individual steps with high divergence due to their differing observation spaces \citep{hu2022policy}. As an example, in a game of football, four players have the role of a defender but, given their observations of the game state and their own positions they would have to react differently to fulfil their assigned roles \citep{kurach2020google}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Task Switching}
\begin{comment}
Based on prior studies, we have established a two-level approach for measuring diversity in task switching. The first level focuses on \textbf{agent action diversity}, which involves tracking the frequency of different actions taken by each agent during evaluation. This information can be used to identify any agents that consistently use the same action or the noop action, indicating laziness, and to assess agent exploration of different actions.

The second level of diversity measurement involves assessing \textbf{agent diversity} by calculating the kl divergence between the action distribution of different agents. By comparing the actions taken by various agents, we can determine whether agents have similar behaviors or different roles. This method enables us to gain insight into the extent of diversity among agents, which can be useful for optimizing task allocation and resource management.
\end{comment}

\begin{comment}
    Task switching is an essential metric for monitoring action usage in multi-agent reinforcement learning (MARL), which allows a thorough examination of the agent's exploration-exploitation balance within its environment, analysis of the agent's learning dynamics, and assessment of diverse learning algorithms and strategies' effectiveness. This metric quantifies the frequency at which an agent selects specific actions..\\

    To track the task switching,  we monitor the usage of each agent action at every timestep $t$ during the evaluation phase of the agent in the training process. By analyzing the recording frequencies, we can compute the likelihood of each action being selected, which we achieve by passing them through a soft-max distribution.  Mathematically it can be described as ...
\end{comment}
By implementing a practical task-switching metric, it becomes possible to quantify the frequency at which an agent selects specific actions during the evaluation phase. This, in turn, enables a thorough examination of the agent's exploration-exploitation balance within its environment, as well as an analysis of the agent's learning dynamics and an assessment of the algorithmic strategy diversity and effectiveness. 

This can be implemented by tracking the usage of each agent action at each timestep $t$ during the evaluation phase of agent training. From the recorded frequencies, we can compute the likelihood of each action being selected by passing the counter through a soft-max distribution to generate a likelihood estimation for each action. Mathematically it can be described as:

\begin{equation}
\mathcal{T}_T = \sigma( \sum^{T}_{t=0} \Vec{a}^{i}_{t})
\end{equation}

Where $\sigma$ is a softmax function used to convert the action counts to a probability distribution, $\Vec{a}^{i}_{t}$ is a one-hot encoded vector of the action chosen by agent $i$ at timestep $t$ and $\mathcal{T}_T$ is a matrix containing the cumulative likelihood of each possible action up until the terminal timestep $T$ for each timestep in the environment $t$.

\begin{comment}
TODO: add equation for kl_div on the probs or just mention it
Monitoring action usage can provide valuable information about the agent learning process in MARL and aid in evaluating the effectiveness of various learning algorithms and strategies. The practical implementation of the task-switching method allows us to measure the frequency an agent takes a specific action during an evaluation phase, allowing us to evaluate the agent's learning to observe how well the agent is exploring-exploiting the environment and to examine the dynamics of the agent's learning.

--------------------------------------------------------------
**Deductions**:

*Learning Dynamics: Tracking action usage provides an indication of how the agent learns. By observing the evolution of action usage over time, we can examine the dynamics of the agent's learning and see whether or not the agent is learning a good policy, so some increase in the usage of actions that lead to higher rewards can be expected.
E.g If an agent's use of actions that result in higher rewards increases, it may imply that the agent is learning an optimal strategy. If, on the other hand, an agent reduces its use of actions that result in lower rewards, it may indicate that the agent is learning to avoid suboptimal behavior.

*Exploration-Exploitation: With the task-switching method we can ensure that the agent explores all possible actions in the environment after each slot of the training phase. This exploration allows the agent to find better policies that result in higher rewards. However, if the agent only explores and never exploits, it may never learn to maximize its rewards.
E.g If an agent consistently chooses the same action, it may be a sign that it's not sufficiently exploring the environment and, therefore, not learning an optimal policy. On the other hand, if an agent explores a wide range of behaviors, it may mean that it is not fully exploiting the best actions and, therefore, not maximizing its rewards.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Agent Contribution}

The ability to directly monitor the contributions of individual agents in a MARL system is critical due to the popularity of value-decomposition algorithms for solving cooperative games. The algorithms like VDN and QMIX rely on improving multi-agent credit assignment to improve agent learning. By analysing this credit assignment it is possible to find new avenues of research to create better decomposition schemes. However, as these methods are typically trained in an end-to-end manner it is difficult to apply explainable deep learning methods to them and explainability is limited to a few explicitly designed algorithms [CTATIONS]. Instead, we explore methods to calculate agent contribution in a manner that is agnostic to the architecture of the algorithm.

\begin{comment}
Understanding each agent's input is critical since it can provide insight into how the agents are learning and behaving in the environment. This knowledge can be used to create more effective learning algorithms. It enables us to find areas for improvement, create better strategies, and encourage collaboration among agents (for example we can mention the algorithms that used the Shapley value to increase performance).

Some ideas why we should consider this contribution/Shapley value:

- it allows us to improve and evaluate the efficiency of the system: By evaluating the performance of each agent, we can evaluate the overall efficiency of the system and identify which agents are performing well (learning an optimal policy) and which ones may be hindering the performance of the group, and we can use this information to make improvements to the system (for example we can adjust the reward structure or modify the behavior of specific agents/ adjust the agents architecture)

-  it helps to understand the behavior of agents: By analyzing the contribution of each agent, we can better understand how agents interact with each other and how they influence their behavior. This information can be used to develop better strategies to achieve the desired outcome and to identify which agents work well together and which do not, and we can take steps to encourage cooperation between agents (reward shaping: adding a positive reward or a penalty for a specific behavior/ distribute the team reward based each contribution).

\end{comment}

\subsubsection{Existing work}
A very famous method used to solve the issue of payoff distribution for the grand coalition is the \textbf{Shapley Value} \citep{shapley1953}. Meaning it it used to determine the contribution of each member of the coalition towards completion of a task. Given a cooperative game $\Gamma = (\mathcal{N},v)$ for any $\mathcal{C} \subseteq \mathcal{N}/\{i\} $ let $\phi_{i}(\mathcal{C}) = v(\mathcal{C} \cup \{i\}) - v(\mathcal{C})$ be a marginal contribution, the Shapley value of each agent $i$ can be written as:
\begin{equation}
Sh_{i}(\Gamma) = \sum_{\mathcal{C} \subseteq \mathcal{N}/\{i\}} \frac{|\mathcal{C}|!(|\mathcal{N}| - |\mathcal{C}|-1)!}{|\mathcal{N}|!} \cdot \phi_{i}(\mathcal{C})
\end{equation}

%Word this better
Where $\mathcal{N}$ is a set of agents, $v$ is the value function used to measure the profits earned by the coalition which maps from a coalition $\mathcal{C} \subseteq \mathcal{N}$. The set of agents $\mathcal{N}$ is also referred to as the grand coalition and contains all agents.

Calculating Shapley values presents two issues, it requires the computation of $2^{n-1}$ possible coalitions of a potential $n(2^{n-1})$  coalitions which is computationally expensive and it requires the use of a simulator where agents can be removed from the coalition and the value of the same states to be evaluated with each coalition.

To make these calculations reasonable, we can instead compute the contributions based on a subset of the coalitions instead of all possible coalitions. We can do this by reformulating the Shapley value calculation as a Monte-Carlo estimate \citep{monte1949}...%Add derivation from paper on notion

This reinterpretation of the Shapley values can be calculated as:
\begin{equation}
\hat{\phi}^{RL}_{i}(r) = \frac{1}{M} \sum^{M}_{m=1}(r^{m}_{+i} - r^{m}_{-i}) \approx \phi_{i}(r)
\end{equation}
Where $\hat{\phi}^{RL}_{i}(r)$ is the shapley value for agent $i$ given joint reward $r$, $M$ is the number of agent in the coalition, $r^{m}_{+i}$ is the return for coalition $m$ out of all possible coalitions $M$ with agent $i$ and $r^{m}_{-i}$ is the return for coalition $m$ out of all possible coalitions $M$ without agent $i$

\subsubsection{Agents importance}
We create an implementation to calculate an online approximation of the shapley value of each agent in the coalition during training time. Importantly our method extends the shapley approximation in \citep{heuillet2021collective} by taking into account the entire coalition of agents at each timesteps. Rather than creating an approximation using the subset of the coalition we create copies of the environment at each timestep equal to the number of agent in the coalition, we then set a unique member of the coalition to use a noop action for each of these parallel environments and calculate the real counterfactual return at each timestep with respect to the missing agent....%Do math here

At each iteration of training, we can then plot these shap approximations using a radial chart where the distance from the center to each edge is the maximum group reward.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training Stability}
\begin{comment}
Understanding the dynamic of a multi-agent reinforcement learning (MARL) system during the learning process is essential for effective and efficient learning. Diagnosing the dynamic of the system can help identify learning instability, slow convergence, and implementation bugs or hyperparameter issues. By being aware of the system's dynamic, we can adjust the learning algorithm or reward function to improve learning and design more robust and effective MARL systems. While our implementation of common methods for measuring training stability may not be considered novel, it is crucial to have them in order to ensure that the learning process is stable and effective.
\end{comment}
\subsubsection{Agent update divergence}
We measure the per step KL divergence of each agent to measure how the policy changes over time. A high KL divergence over time is usually indicative of a stochastic policy and can be thought of as a measurement of agent stability or if the agent policy has converged to an optimal parameterisation. KL Divergence can also be measured on a per agent basis and compared. If individual agents have high KL divergence and other do not, it can indicate a tendency for the MARL policy to overweight certain agents in the coalition and learn unbalanced policies.

\subsubsection{Team and individual entropy}
It was shown by \cite{abdallah2009global} that using only the global returns as a metric may hide underlying instability in agent policies. They suggest using the agent policy entropy as a proxy for measuring the stability with which an agent $i$ has converged to a certain behaviour. This can be computed as for each agent as 

\begin{equation}
H_i(\pi( \cdot | o^i_t)) = - \sum_{a^i \in A^i} \pi(a^i|o^i_t) \log \pi(a^i|o^i_t))    
\end{equation}

Where $i$ is the id of an individual agent in the coallition, $o$ is an individual agent observation, $a^i$ is the action of agent $i$ at timestep $t$, $\pi$ is the policy of agent $i$ and $H_i$ the entropy of agent $i$. This is extended to the full team by computing the mean team entropy as 

\begin{equation}
%H(\pi( \cdot | o_i, \dots, o_n)) = \mathbb{E}[H_i]    
H(\pi( \cdot | o_i, \dots, o_n)) = \frac{1}{n}\sum^n_{i=0} H_i  
\end{equation}
Where $n$ is the total number of agents in the coalition.


==> sections/previous_work/3-experiment_draft.tex <==
\section{Experiments}

\citep{papoudakis2021benchmarking} perform a thorough evaluation sweep with common MARL algorithms to generate comparative insights into relative algorithmic performance. The comparative performance across four different settings revealed a flaw in MARL benchmarking which is dominated by SMAC and MPE. The authors found that the performance rankings on SMAC and MPE do not translate into all types of settings. In particular they make use of LBF and RWARE as additional benchmarks which provided new insights that would have been previously overlooked. We perform an additional analysis into these two settings to discover why certain algorithms produce anomalous results in certain cases.

\subsection{Environments}

From their evaluation, the results that are the most unexpected are those found on RWARE and LBF. Given that limitations with prior baselines were already discovered in these two settings, we make them the focus of our analysis.

\textbf{Multi-Robot Warehouse (RWARE)} is a multi-agent environment, that is designed to represent a simplified setting where robots move goods around a warehouse. The environment requires agents (circles) to move requested shelves (coloured squares) to the goal post ('letter' G) and back to an empty room as illustrated in figure \ref{fig:rware} below. It is a partially observation setting with a very sparse reward signal as agents have a limited field of view are are rewarded only on a successful delivery \citep{christianos2020shared, christianos2021scaling}.

\textbf{Level-Based Foraging (LBF)} is a mixed cooperative-competitive game with a focus on inter-agent coordination illustrated in figure \ref{fig:lbf} below. Agents of different skill levels navigate a grid world and collect food by cooperating with other agents if required. Agents placed in the gridworld are assigned a level and can only collect food if the sum of the agent levels involved is at least equal to the level of the food. Agents are awarded point equal to the level of the collected food divided by their level \citep{albrecht2015gametheoretic, albrecht2019reasoning, christianos2020shared}. There is also a purely cooperative version. We report findings in both settings.


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/Rware.png}
        \caption{RWARE}
        \label{fig:rware}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/LBF.png}
        \caption{Level Based Foraging (LBF)}
        \label{fig:lbf}
    \end{subfigure}
    \caption{Example visualisation for the RWARE and LBF settings}
    \label{fig:rware_lbf}
\end{figure}

\subsection{Algorithms}

For our analysis we make use of a limited subset of the existing algorithms in the MARL literature. We select these algorithms.These algorithms cover Deep Q-Learning (DQL), policy-gradient (PG), centralised training decentralised execution (CTDE) and independent learning (IL) methods. Given a common taxonomy of SARL algorithms it is reasonable to group the majority of algorithms as either value or policy based \citep{zhang2020taxonomy, canese2021multi}. From this taxonomy the most successful value-based methods have been developed from improvements to the DQL algorithm and policy-based methods from variants of policy gradient algorithms like REINFORCE \citep{REINFORCE}. Additionally, given that we only explore cooperative MARL settings it is reasonable to investigate the CTDE vs IL paradigm as CTDE methods expand SARL methods for MARL settings and have become the common strategy for solving cooperative MARL problems. For our study we make up of Independent Q-Learning (IQL), Value-Decomposition Network (VDN) and QMIX covering off-policy algorithms and Multi-Agent Proximal Policy Optimisation (MAPPO) and Multi-Agent Advantage Actor-Critic (MAA2C) covering on-policy methods.


\subsection{Evaluation Protocol}
We follow the protocol outlined by \citep{gorsane2022standardised} which applies the tools from \citep{agarwal2022deep} to the MARL setting. The \textbf{evaluation parameters} used are 2 million training timesteps for off-policy algorithms and 20 million for on-policy to account for sample efficiency, 10 independent training runs with 32 evaluation episodes per interval at every 10000 timesteps...

\subsection{Case Studies}

We enhance the data from \citep{papoudakis2021benchmarking} on the LBF and RWARE settings by incorporating the robust metrics proposed by \citep{agarwal2022deep}. Using the MARL evaluation toolset provided by \citep{gorsane2022standardised}, we provide a more comprehensive overview of their findings. The necessity of this reanalysis stems from recent literature, highlighting the limitations and high experimental variance in traditional empirical performance measurements [emarl citations]. We employed the same hyperparameters as in\citep{papoudakis2021benchmarking}, with a complete summary of our findings available in Appendix B. From this reanalysis.

Our reevaluation shows the same algorithmic rankings across various aggregation methods, as shown in figures \ref{fig:aggregations_rware} and \ref{fig:aggregations_lbf}. No change in relative ranking was observed when using the interquartile mean, absolute metric or performance profiles. This consistency validates that the outliers are not artifacts of evaluation protocols, emphasizing the need for understanding agent behavior during or post-training for diagnosing such inconsistencies.

\textbf{Case 1: } Figure \ref{fig:aggregations_rware} illustrates that in RWARE, irrespective of aggregation method, fail to achieve high returns. Given the difficulty of value-decomposition in sparse settings, it is expected for methods like VDN and QMIX to perform sub-optimally when most returns are zero \citep{mahajan2019maven}[More Citations for SParsity]. Despite this, both VDN and QMIX have shown some capacity to learn some sparse settings \citep{mguni2022ligs} and IQL occasionally discovers policies that can solve complex parse settings in the MARL domain \citep{mahajan2019maven}. Therefore, it becomes crucial to identify if agent policies have prematurely converged to low-reward policies using \textit{agent update divergence} and compare \textit{state visitations} to understand the trajectories of the agents.

\begin{figure}[h]
  \centering
\includegraphics[width=0.7\textwidth]{figures/rware_return_aggregate_scores.png}
  \caption{Aggregations of RWARE returns on baseline algorithms}
  \label{fig:aggregations_rware}
\end{figure}

\begin{figure}[h]
  \centering
\includegraphics[width=\textwidth]{figures/lbforaging_return_aggregate_scores.png}
  \caption{Aggregations of LBF returns on baseline algorithms}
  \label{fig:aggregations_lbf}
\end{figure}
\textbf{Case 2:}The LBF setting presents an unusual performance trend when comparing the PPO and A2C algorithms, as shown in Figure \ref{fig:lbf_performance_profile}.  Contrary to usual expectations of PPO methods performing at least as well as A2C methods, both IA2C and MA2C surpass MAPPO and IPPO. PPO is often seen to outperform A2C in the majority of SARL and MARL literature \citep{schulman2017proximal, garg2021proximal}. It is noteworthy that in LBF MAPPO not conly converges more slowly but also to a less-optimal final policy than MAA2C despite it's typically higher sample efficiency.

This performance disparity isn't as straightforward as RWARE's sparsity, but we leverage behavior analysis metrics to shed light on it. Similar to Case 1, we utilize \textit{state visitation} to observe if particular states are preferred early in training, and \textit{agent importance} to discern any overreliance on specific agents. Further, we analyze \textit{team and individual agent entropy} to evaluate whether MAA2C policy has settled into a stable optima and if MAPPO has converged to a local optima or remains unstable due to hyperparameters.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/rware_performance_profile.png}
        \caption{Algorithm performance profiles on RWARE}
        \label{fig:rware_performance_profile}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/lbforaging_performance_profile.png}
        \caption{Algorithm performance profiles on LBF}
        \label{fig:lbf_performance_profile}
    \end{subfigure}
    \caption{Algorithm performance profiles for baseline algorithms on RWARE and LBF showing the likelihood of algorithms to reach different levels of minimum performance}
    \label{fig:rware_lbf_performance_profiles}
\end{figure}

\textbf{Case 3: }Figure \ref{fig:rware_sup} showcases another RWARE anomaly, where IQL demonstrates a high probability to outperform both VDN/QMIX. This finding contrasts with most cooperative settings, where IQL typically performs slower and converges to less optimal policies compared to its value-decomposition counterparts \citep{SMAC}[citation]. 

To understand this anomaly, we contrast performances on cooperative and mixed LBF settings to examine why VDN and QMIX underperform in this setting. Our analysis leverages \textit{task-switching} to display algorithmic tendency towards ineffective actions, and \textit{agent contributions} to demonstrate errors in sparse credit assignment.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/rware_return_prob_of_improvement.png}
        \caption{The probability of algorithmic superiority for base line algorithms on RWARE}
        \label{fig:rware_sup}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/lbforaging_return_prob_of_improvement.png}
        \caption{The probability of algorithmic superiority for base line algorithms on LBF}
        \label{fig:lbf_sup}
    \end{subfigure}
    \caption{Algorithm performance profiles for baseline algorithms on RWARE and LBF showing the likelihood of algorithms to reach different levels of minimum performance}
    \label{fig:rware_lbf_sup}
\end{figure}



\subsection{Error detection}
To demonstrate the utility of interpretability tools in MARL algorithm development, we incorporate typical challenges in practical MARL implementations into the epymarl framework. We highlight how these issues can be detected in LBF and RWARE settings using behavior explanation.

Hyperparameter tuning is a persistent challenge in both SARL and MARL. Similar to SARL, standard MARL algorithms do not self-tune their hyperparameters and manuallyed tuned algorithms are limited to a small set of optimal parameters \citep{jordan2020evaluating}. This limitation is also present in MARL when performing inter-algorithmic comparisons \citep{hu2022rethinking}. Though researchers often conduct a hyperparameter sweep to identify a suitable range of parameters, this approach may not always be feasible or exhaustive, particularly for slow simulators or highly complex algorithms.

\begin{table}[H]
\centering
\caption{A table of permutations of hyperparameters that will be tested}
\label{tab:permutation}
\begin{tabular}{@{}lllllll@{}}
\toprule
Algorithm & epsilon anneal & PPO-CLIP & Target Update & n-step & Learning Rate & Lambda \\ \midrule
IQL       & 1              & -        & 1             & 1      & 1             & 1      \\
MAPPO     & -              & 1        & 1             & 1      & 1             & 1      \\ \bottomrule
\end{tabular}
\end{table}

In table \ref{tab:permutation} we list all permutations of hyperparameters to be tested. Taking inspiration from \citep{hu2022rethinking}, we focus on learning rates and training batch sizes. We test for three values of each; a value that is below the accepted range, the standard in literature and one that is above the normal range.


We also show that our metrics can be used to diagnose common implementation errors which can lead to "silent failure" in MARl applications. A simply but common "silent failure" case is incorrect terminal state masking \citep{yu2022surprising}. To achieve high performance when using on-policy algorithms in environments without a fixed rollout lengths it is important to remove the gradient calculations associated
with padded data for batch training. If this not done then the algorithm will still learn but often converge to a suboptimal policy. We show that the need for masking can be determined using \textit{agent importance} and \textit{task switching}. If padding data is being used during training it is reasonable to assume the algorithm will become destabilised by learning to interpret the fake data. In figure X below, we can see if an algorithm is able to converge in a setting, task probability over time will naturally converge at a point that correlates with a stable policy irrespective of the optimality of that policy. In cases where masking is not used, the algorithms will develop divergent policies over time.






==> sections/previous_work/3-experiments.tex <==
\section{Experiments}

\citep{papoudakis2021benchmarking} perform a thorough evaluation sweep with common MARL algorithms to generate comparative insights into relative algorithmic performance. The comparative performance across four different settings revealed a flaw in MARL benchmarking which is dominated by SMAC and MPE. The authors found that the performance rankings on SMAC and MPE do not translate into all types of settings. In particular they make use of LBF and RWARE as additional benchmarks which provided new insights that would have been previously overlooked. We perform an additional analysis into these two settings to discover why certain algorithms produce anomalous results in certain cases.

\subsection{Environments}

From their evaluation, the results that are the most unexpected are those found on RWARE and LBF. Given that limitations with prior baselines were already discovered in these two settings, we make them the focus of our analysis.

\textbf{Multi-Robot Warehouse (RWARE)} is a multi-agent environment, that is designed to represent a simplified setting where robots move goods around a warehouse. The environment requires agents (circles) to move requested shelves (coloured squares) to the goal post ('letter' G) and back to an empty room as illustrated in figure \ref{fig:rware} below. It is a partially observation setting with a very sparse reward signal as agents have a limited field of view are are rewarded only on a successful delivery \citep{christianos2020shared, christianos2021scaling}.

\textbf{Level-Based Foraging (LBF)} is a mixed cooperative-competitive game with a focus on inter-agent coordination illustrated in figure \ref{fig:lbf} below. Agents of different skill levels navigate a grid world and collect food by cooperating with other agents if required. Agents placed in the gridworld are assigned a level and can only collect food if the sum of the agent levels involved is at least equal to the level of the food. Agents are awarded point equal to the level of the collected food divided by their level \citep{albrecht2015gametheoretic, albrecht2019reasoning, christianos2020shared}. There is also a purely cooperative version. We report findings in both settings.


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/Rware.png}
        \caption{RWARE}
        \label{fig:rware}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/LBF.png}
        \caption{Level Based Foraging (LBF)}
        \label{fig:lbf}
    \end{subfigure}
    \caption{Example visualisation for the RWARE and LBF settings}
    \label{fig:rware_lbf}
\end{figure}

\subsection{Algorithms}

For our analysis we make use of a limited subset of the existing algorithms in the MARL literature. We select these algorithms.These algorithms cover Deep Q-Learning (DQL), policy-gradient (PG), centralised training decentralised execution (CTDE) and independent learning (IL) methods. Given a common taxonomy of SARL algorithms it is reasonable to group the majority of algorithms as either value or policy based \citep{zhang2020taxonomy, canese2021multi}. From this taxonomy the most successful value-based methods have been developed from improvements to the DQL algorithm and policy-based methods from variants of policy gradient algorithms like REINFORCE \citep{REINFORCE}. Additionally, given that we only explore cooperative MARL settings it is reasonable to investigate the CTDE vs IL paradigm as CTDE methods expand SARL methods for MARL settings and have become the common strategy for solving cooperative MARL problems. For our study we make up of Independent Q-Learning (IQL), Value-Decomposition Network (VDN) and QMIX covering off-policy algorithms and Multi-Agent Proximal Policy Optimisation (MAPPO) and Multi-Agent Advantage Actor-Critic (MAA2C) covering on-policy methods.


\begin{comment}
 \subsubsection{Deep Q-Learning (DQL)}


\textbf{IQL:} For Independent Q-Learning (IQL) \citep{tan1993multi}, each agent learns a policy based purely on their own egocentric experience in the training environment. This policy is parameterised by a Q-value network \citep{mnih2013playing}.

\textbf{VDN:} In Value-Decomposition Network (VDN) \citep{sunehag2017value}, IQL is extended through the use of value decomposition. Rather than learning purely from their own egocentric perspectives with each agent receiving the same reward, VDN formulates the joint Q value of the coalition as a linearly decompose sum of the individual agent values. Each IQL agent then learns using the gradient flow based on a joint additive loss.

\textbf{QMIX}: \citep{rashid2018qmix} then extends VDN by broadening the range of reward functions that can be decomposed. To create a more complex attribution of the Q values, it makes use of a parameterised mixing network to perform the attribution. This mixing network takes the IQL agent Q values as input and then learning is performed in an end-to-end manner where attribution is done using backpropagation. Qmix also allows the use of data augmentation by accommodating additional data at training time. 

\subsubsection{Policy Gradients (PG)}

\textbf{IA2C:} Independent Advantage Actor-Critic (IA2C) is a variant of the A2C algorithm \citep{pmlr-v48-mniha16} applied to the multi-agent setting. IA2C trains agents using their own egocentric experiences in the training environment where each agent has their own critic and actor networks which approximate the optimal policy and state values.

\textbf{IPPO:} Independent Proximal Policy Optimisation (IPPO) is a variant of the PPO algorithm \citep{schulman2017proximal} applied to the multi-agent setting. PPO can be thought of as an improvement to A2C. It used a surrogate objective which limits the change in the policy at each update step, this allows PPO to iterate over the same trajectory of data multiple times without policy divergence. Otherwise its architecture is the same as A2C.

\textbf{MAPPO \& MAA2C:} Multi-Agent Proximal Policy Optimisation (MAPPO) and Multi-Agent Advantage Actor-Critic (MAA2C) \citep{yu2022surprising} extend IPPO and IA2C to make use of a joint state value function. Instead of multiple per agent critics, there is a single critic that learns the value of the joint state representation rather than the egocentric individual agent observations. MAA2C is also sometimes referred to as Central-V \citep{foerster2018counterfactual} because of this but, to prevent confusion we use MAA2C and MAPPO also makes use of the same architecture.   
\end{comment}


\subsection{Evaluation Protocol}
We follow the protocol outlined by \citep{gorsane2022standardised} which applies the tools from \citep{agarwal2022deep} to the MARL setting. The \textbf{evaluation parameters} used are 2 million training timesteps for off-policy algorithms and 20 million for on-policy to account for sample efficiency, 10 independent training runs with 32 evaluation episodes per interval at every 10000 timesteps...
\subsection{Case Studies}

On the RWARE and LBF settings, we enhance the data from \citep{papoudakis2021benchmarking} by using an additional set of more robust metrics proposed by \citep{agarwal2022deep} using the MARL evaluation toolset provided by \citep{gorsane2022standardised} to provide clearer insight into the original findings from these settings. This reanalysis is done to ensure consistent performance rankings as recent literature has found traditional empirical performance measurements to have limited robustness and high variance between experiments [emarl citations]. For these experiments we reuse the hyperparameters from \citep{papoudakis2021benchmarking}. The full summary of this reanalysis can be found in Appendix B. From this reanalysis, algorithmic rankings are unchanged when using multiple aggregation methods show in figures \ref{fig:aggregations_rware} and \ref{fig:aggregations_lbf}.

From this reanalysis, relative algorithmic rankings are unchanged when we use both the interquartile mean, absolute metric and the performance profiles. This confirms that the anomalous results are not a byproduct of evaluation protocols and in order to diagnose these issues it is important to be able to explain the algorithmic behavior of the agents either during or after training.

\textbf{Case 1: }In figure \ref{fig:aggregations_rware} below we can see that in RWARE, all value-iterations methods are unable to achieve a return much greater than zero irrespective of the aggregation method used. It is expected for value-iteration methods, especially VDN and QMIX to have reduced performance in sparse settings as it is difficult to perform value-decomposition when the majority of returns are zero \citep{mahajan2019maven}[More Citations for SParsity]. However both VDN and QMIX have shown the a limited capacity to learn some sparse settings \citep{mguni2022ligs} and IQL is in some cases able to find polices that can solve high complexity sparse settings in the MARL domain \citep{mahajan2019maven}. 

\begin{figure}[h]
  \centering
\includegraphics[width=\textwidth]{figures/rware_return_aggregate_scores.png}
  \caption{Aggregations of RWARE returns on baseline algorithms}
  \label{fig:aggregations_rware}
\end{figure}

\begin{figure}[h]
  \centering
\includegraphics[width=\textwidth]{figures/lbforaging_return_aggregate_scores.png}
  \caption{Aggregations of LBF returns on baseline algorithms}
  \label{fig:aggregations_lbf}
\end{figure}
\textbf{Case 2:}In LBF we find anomalous performance with respect to the comparative performance of the PPO and A2C based methods as illustrated in the performance profiles in figure \ref{fig:lbf_performance_profile}. Both IA2C and MA2C outperform MAPPO and IPPO however, we would usually assume that PPO methods at minimum perform as poorly as A2C methods and in the majority of both SARL and MARL literature PPO will achieve better performance than A2C in common settings \citep{schulman2017proximal, garg2021proximal}. More interesting is that the PPO methods seem to have slower converge as well as converging to a poorer final policy than the A2C methods as PPO typically also has higher sample efficiency. This gap in performance is not as intuitive as the sparsity of RWARE but, we are able to discover insights that explain this anomaly using the behavior analysis metrics. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/rware_performance_profile.png}
        \caption{Algorithm performance profiles on RWARE}
        \label{fig:rware_performance_profile}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/lbforaging_performance_profile.png}
        \caption{Algorithm performance profiles on LBF}
        \label{fig:lbf_performance_profile}
    \end{subfigure}
    \caption{Algorithm performance profiles for baseline algorithms on RWARE and LBF showing the likelihood of algorithms to reach different levels of minimum performance}
    \label{fig:rware_lbf_performance_profiles}
\end{figure}

\textbf{Case 3: }Another anomaly on RWARE the performance of VDN/QMIX when compared to IQL, in figure \ref{fig:rware_sup} we can see there is a high probability for IQL to outperform both value-decompositon algorithms. On most cooperative settings IQL is slower and converges to worse polices than the value-decomposition counterparts \citep{SMAC}[citation] which is not reflected in this setting. We compare performance on the cooperative and mixed LBF settings and explain why VDN and QMIX seem to experience degraded performance on this setting.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/rware_return_prob_of_improvement.png}
        \caption{The probability of algorithmic superiority for base line algorithms on RWARE}
        \label{fig:rware_sup}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/lbforaging_return_prob_of_improvement.png}
        \caption{The probability of algorithmic superiority for base line algorithms on LBF}
        \label{fig:lbf_sup}
    \end{subfigure}
    \caption{Algorithm performance profiles for baseline algorithms on RWARE and LBF showing the likelihood of algorithms to reach different levels of minimum performance}
    \label{fig:rware_lbf_sup}
\end{figure}


\begin{comment}
    \subsection{Agent Importance}
As mentioned in section 2.1, we create an implementation to calculate an online approximation of the shapley value of each agent in the coalition during training time. Importantly our method extends the shapley approximation in \citep{heuillet2021collective} by taking into account the entire coalition of agents at each timesteps. Rather than creating an approximation using the subset of the coalition we create copies of the environment at each timestep equal to the number of agent in the coalition, we then set a unique member of the coalition to use a noop action for each of these parallel environments and calculate the real counterfactual return at each timestep with respect to the missing agent....%Do math here

At each iteration of training we can then plot these shap approximations using a radial chart where the distance from the center to each edge is the maximum group reward. In figure \ref{fig:shape_values_per_agent} we can see that once an optimal policy has been reached it is typical for the shap contributions per agent to be fairly equal. Before agents have reached an equilibrium the workload is distributed unevenly and without coordinate the environments cannot be solved effectively...

\begin{figure}[h]
  \centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/placeholder.jpeg}
\caption{Radar plots}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/placeholder.jpeg}
\caption{Line plots over time}
\label{fig:subim2}
\end{subfigure} 
  \caption{Shapley values per agent.}
  \label{fig:shape_values_per_agent}
\end{figure}

\subsection{Agent Task Switching}
Over the course of training we can track agent policies and track the frequency individual actions over time. Naturally we assume the policies should become more deterministic over training time...

We can combine this with a measurement of the joint policy entropy over time. This can be used to diagnose policy collapse, when agents reach a high reward joint policy but entropy is still high it is possible for agents to re-converge to a suboptimal policy...

\subsection{Algorithmic Stability}
We measure the per step KL divergence of each agent to measure how the policy changes over time...

Measure the KL divergence between agents with and without parameter sharing and show that it can be used to diagnose when to use shared or split parameters...

\subsection{Policy Diagnosis}

The work done in \citep{papoudakis2021benchmarking} shows the performance of MARL algorithms in certain cases do not match with common assumptions in literature. More specifically in LBF, both IA2C and MAA2C outperform IPPO and MAPPO which are usually superior in most cases and IQL out performs both VDN and QMIX...

In RWARE[cite] the value iteration algorithms are completely unable to learn...

We perform an ablation on these two settings using all of the metrics mentioned in the paper while altering hyperparameters and introducing common failure points into the epymarl framework...

From the results below we show that policy diagnosis metrics are able to reveal more clearly when there are issues in the implementation of the MARL algorithms...
\end{comment}

\subsection{Metric Use Case}

Here we detail the application of the proposed metrics in each case study with the goal of creating explanations linking the empirical performance of MARL algorithms to their theoretical foundations.

\textbf{Case 1: } In case 1 the primary anomaly is the DQL based agents all receive a return of 0 across all training steps. It is reasonable to assume this is due to sparse rewards but, even with sparse rewards, given the appropriate exploration parameterisation it should be possible to achieve a reward that is greater than 0. Given this assumption it is important to determine if the DQL agents are prematurely converging before enough environment exploration is done. We can measure this using the \textit{agent update divergence} metric to determine if the agent policies are prematurely converging and then track \textit{state visitations} against this to see if the policy becomes overly deterministic before exploring all of the options present on the map.

%The idea is PPO updates create early estimations of the optimal state which are not correct and this guides exploration in a suboptimal manner. Idk the paragraph is worded weirdly -Siddarth
\textbf{Case 2: } In case 2 MAA2C outperforms MAPPO by a wide margin, which does not match the findings in most settings. Given that the core architecture of PPO extends A2C by adding the clipping function, we can assume that the reduced performance is due to the additional update steps moving MAPPO into an early suboptimal policy, which then reduces effectiveness for the rest of training. The fact that MAPPO also converges more slowly than MAA2C in LBF supports this hypothesis, as PPO should be utilising data more efficiently. 

For this case we want to measure the tendency of the algorithms to learn to overvalue states early in training, given that unlike IQL, methods PG methods use the agent policy to guide exploration. Like in \textbf{case 1}, we make use of \textit{state visitation} to determine if there is a tendency to favor certain states early in training. We also make use of \textit{agent importance} to determine if these additional updates are creating polices that favor certain agents at the detriment of the joint policy. Additionally, we examine \textit{team and individual entropy} to determine if, after training to completion, the MAA2C policy is as stable as it appears and if MAPPO has fully converged to the suboptimal policy or if the joint policy is unstable and could be improved suing hyperparameter optimisation.


% We could also use joint entropy to check if algorthms have actually converges after the graphs cut off. Maybe it's reasonable to explain it as agents can sometimes learn slowy or have big jumps in performance and since we don't have infinite time it would be useful to check? - Siddarth
\textbf{Case 3: }Finally, in case 3, we find that IQL outperforms both VDN and QMIX. In the cooperative setting, this is highly uncommon, and although it can occur in individual scenarios, it is unexpected to be common across multiple scenarios from the same benchmark. We assume this is due to LBF allowing for selfish actions, which can be detrimental to the global reward, creating global value functions that take longer for QMIX and VDN to properly decompose into per-agent rewards. The results on LBF support this, as all three algorithms seem to converge to a similar final reward, but QMIX and VDN have slower initial learning curves.

Using agent importance, we measure the individual agent contributions to the coalition during training to show that QMIX and VDN are misprioritizing agents during updates, and their performance reduction compared to IQL is a byproduct of the reward structure of LBF.

\subsection{Policy Diagnosis}

To collect the data to run our behavior explanation metrics we rerun the experiments on LBF and RWARE using the same hyperparameters as \citep{papoudakis2021benchmarking}. The only change is increasing he number of seeds used to 10 from the 5 of the original paper. We then store the data from these runs in JSON files which will be made available as a public dataset[LINK]. This dataset contains the full environment rollouts from all evaluation steps done during training, environment returns and the results of the online and offline data analysis using the metrics from section 2.

The online values calculated are our agent contribution calculation and the shapley values at each timestep. These are built into a general library which can be added into existing frameworks. As these values need to be calculated during runtime and multiple deep learning frameworks exist, this library requires data to be converted to a compatible type before it is used.

Offline values are the calculations of team and individual entropy, agent update divergence, task switching and action based role. Our framework does allow for these algorithms to be calculated online however, it is more efficient to calculate this suite of values offline to ensure that training speed is not impacted. For gridworld-based settings like RWARE and LBF the environments step quickly enough that online calculations make a noticeable change in training time.

\subsection{Error detection}
To show the value of policy diagnosis in creating MARL algorithms, we introduce common issues with practical MARL implementations into the epymarl framework and show how in LBF and RWARE, these issues can be detected using behavior explanation.


A difficulty in both SARL and MARL in hyperparameter tuning. Common MARL algorithms, much like in SARL do not auto-tune their own hyperparameters and manually tuned algorithms tend to only perform well on a small set of optimal settings \citep{jordan2020evaluating}. In MARL this has also been shown to be true when trying to compare the optimal performance between algorithms \citep{hu2022rethinking}. Authors will usually attempt a hyperparameter sweep to find some range of acceptable parameters but, this is not always possible or comprehensive for slower simulators or very complex algorithms. 

\begin{table}[H]
\centering
\caption{A table of permutations of hyperparameters that will be tested}
\label{tab:permutation}
\begin{tabular}{@{}lllllll@{}}
\toprule
Algorithm & epsilon anneal & PPO-CLIP & Target Update & n-step & Learning Rate & Lambda \\ \midrule
IQL       & 1              & -        & 1             & 1      & 1             & 1      \\
MAPPO     & -              & 1        & 1             & 1      & 1             & 1      \\ \bottomrule
\end{tabular}
\end{table}

In table \ref{tab:permutation} we list all permutations of hyperparameters to be tested. In each entry the center value in bold is consistent with the values used in literature. When choosing the suboptimal parameters we generally still use values that are not excessively out of a reasonable range. Essentially we test values that could be misused by a researcher and take inspiration from \citep{hu2022rethinking}. In our results we show how mistuned hyperparameters produce consistent results when agent behavior is measured.

We also use our metrics to diagnose common implementation errors which can lead to "silent failure" in MARL applications. Two simple  "silent failure" cases are Generalised Advantage Estimation (GAE) \citep{schulman2015high} indexing and incorrect agent masking \citep{yu2022surprising}. GAE is commonly used in A2C and PPO implementations as a method to calculate the training loss, in practical implementations it is possible to index the per step rewards one step off from intended which can cause agents to be unable to learn but still produce a minimisable loss function which creates the appearance of training. Using \textit{team and individual entropy} (TIE) we can measure the instability of the system to determine if the GAE loss being used is updating the correct states associations. When the indexing is incorrect there will be commonly occurring spikes in the TIE measure as policy is being optimised using an incorrect loss that does not correspond to the correct state-reward mappings. Similarly to achieve high performance when using on-policy algorithms in SMAC, it is important to remove the gradient calculations associated with dead agents, if this not done then the algorithm will still learn but often converge to a suboptimal policy. In both of these cases these issues cannot be diagnosed easily by looking into the NN data from training like policy loss overtime. We show that the need for masking can be determined using \textit{agent importance} and \textit{agent update divergence} (AUD). Given that certain agents are removed from the environment at certain steps it is reasonable to assume their contribution to the joint policy while removed is zero. \textit{Agent importance} shows that in the MARL system there are agents that have no effect on the joint policy over multiple steps. We can then assume that these agents must be masked out and not trained on. Additionally when masking is not used the MARL system will attempt to assign value to irrelevant agents which will cause their policies and the joint policy to change over time even when it seems to have converged to a fixed reward. We can make use of AUD to track the individual update magnitudes over time. If there are agents that still have a high AUD after empirical return has stabilised it can be assumed there are redundant agents that need to accomadated during training.






==> sections/previous_work/4-discussion.tex <==
\section{Discussion}

% It would make sense to check which metrics are correlated vs uncorrelated with the returns. 
% If we find a metric that is decoupled from the team return we cold argue that this could be used to measure behaviour / debug a system regardless of the return. 


\textbf{How effectively do empirical returns provide a holistic picture of algorithmic performance?}. The benchmarking process in MARL primarily depends on the empirical return of agents. Although robust statistical methods have been introduced over time, they are still reliant on return for insights into agent behavior. In \textbf{case 1}, the empirical return suggests that Q-learning based methods are completely unable to learn in the RWARE setting. \citep{papoudakis2021benchmarking} reasonably attributes this to the sparsity of the setting, which limits the potential of Q-learning algorithms. However from only empirical returns, the aspect of the sparsity causing these training issues is not apparent.

When measuring \textit{task switching} in figure \ref{fig:iql_mappo_rware}, it is clear that RWARE relies in specific high importance actions that the agent must learn to exploit, therefore the problem is not only reward sparsity but also action relevance. Essentially, Q-learning methods struggle to learn because the environment is disadvantageous for the random data sampling using to train DQNs. This is reflected in the plots of the \textit{joint-entropy} in figure \ref{fig:iql_mappo_rware_ent} where IQL does briefly show a reduction in entropy where is is beginning to learn to exploit the reward while MAPPO has learnt a strongly deterministic policy.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/iql_rware-small-4ag-v1_task_switching.png}
        \caption{Measurement of task switching for IQL on RWARE}
        \label{fig:rware_task}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/mappo_rware-small-4ag-v1_task_switching.png}
        \caption{Measurement of task switching for MAPPO on RWARE}
        \label{fig:lbf_task}
    \end{subfigure}
    \caption{Comparison of task-swithcing for MAPPO and IQL on the RWARE setting}
    \label{fig:iql_mappo_rware}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/iql_rware-small-4ag-v1.png}
        \caption{Measurement of joint-entropy for IQL on RWARE}
        \label{fig:rware_ent}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/mappo_rware-small-4ag-v1.png}
        \caption{Measurement of joint-entropy for MAPPO on RWARE}
        \label{fig:lbf_ent}
    \end{subfigure}
    \caption{Comparison of joint-entropy for MAPPO and IQL on the RWARE setting}
    \label{fig:iql_mappo_rware_ent}
\end{figure}

\begin{comment}
Employing \textit{task-switching}, we observe that PPO prioritizes certain actions excessively early in training, constraining exploration and lowering the maximum achievable return to a local minimum. This observation is confirmed by the KL-Divergence over training (Figure \ref{fig:maa2c_mappo_lbf}), where MAPPO's divergence between training iterations becomes over ten times lower than MAA2C quite early.

By tracking \textit{state-visitations}, we find that PPO tends to prioritize a smaller subset of states much earlier than A2C, failing to thoroughly explore the space. This trend is mirrored in the empirical returns, as MAPPO follows a similar learning trajectory as A2C, oscillating between suboptimal rewards rather than converging. However, measuring the \textit{joint-entropy} in Figure \ref{fig:maa2c_mappo_lbf} verifies that the PPO policy has indeed become fairly deterministic, and despite the oscillation in return usually viewed as instability, the policy is actually stable at a suboptimal setting.

In essence, while empirical return is a useful measure of raw agent performance, it falls short of providing a holistic understanding of agent behavior. Without additional metrics, it does not provide researchers with sufficient insights into MARL algorithms' limitations, preventing the discovery and solution of new challenges.
\end{comment}

In \textbf{Case 2}, the empirical returns show an anomaly where PPO is outperformed by A2C, contrary to the common assumption that PPO should, at minimum, match A2C in performance. These returns only reflect algorithm rankings, failing to explain why such an anomaly occurs.

Using \textit{task-switching} , we observe that PPO over-prioritises certain actions early in training, constraining exploration and limiting the maximum achievable return to a local minima. This observation is confirmed by the KL-Divergence over training (Figure \ref{fig:maa2c_mappo_lbf}), where MAPPO's divergence between training iterations becomes over ten times lower than MAA2C quite early.


By tracking \textit{state-visitations}, we find that PPO tends to prioritize a smaller subset of states much earlier than A2C and does not fully explore the space. This is reflected in the empirical returns as MAPPO follows a similar learning trajectory to A2C but seems to oscillate between suboptimal rewards rather than converging. However, measuring the \textit{joint-entropy} in figure  \ref{fig:maa2c_mappo_lbf} verifies that the PPO policy has become fairly deterministic and despite the oscillation in return which is commonly seen an instability the policy is actually stable at a suboptimal minima. 

In essence, while empirical return is a useful measure of raw agent performance, it falls short of providing a holistic understanding of agent behavior. Without additional metrics, it does not provide researchers with sufficient insights into MARL algorithms' limitations and obscures potential avenues of research.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/maa2c_Foraging-15x15-3p-5f-v2_kl_divergence.png}
        \caption{Measurement of KL-Divergence for MAA2C on LBF}
        \label{fig:lbf_maa2c_kl}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/mappo_Foraging-15x15-3p-5f-v2_kl_divergence.png}
        \caption{Measurement of KL-Divergence for MAPPO on LBF}
        \label{fig:lbf_mappo_kl}
    \end{subfigure}
    \caption{Comparison of KL-Divergence for MAPPO and MAA2C on the LBFE setting}
    \label{fig:maa2c_mappo_lbf}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/maa2c_Foraging-15x15-3p-5f-v2.png}
        \caption{Measurement of joint-entropy for MAA2C on LBF}
        \label{fig:lbf_maa2c_ent}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/mappo_Foraging-15x15-3p-5f-v2.png}
        \caption{Measurement of joint-entropy for MAPPO on LBF}
        \label{fig:lbf__mappo_ent}
    \end{subfigure}
    \caption{Comparison of joint-entropy for MAA2C and MAPPO on the LBF setting}
    \label{fig:maa2c_mappo_lbf_ent}
\end{figure}

In \textbf{case 3} the \textit{agent importance} from figure \ref{fig:iql_qmix_rware_imp} has higher variance over the course of training for VDN and QMIX. Given that value-decomposition is functionally decomposing rewards using agent relevance, we can assume that the poor performance it due to sub-optimal credit assignment. Interestingly VDN does not perform significantly poorer than IQL and when measuring \textit{task switching} we can see that it follows a similar trajectory during training. However, QMIX overprioritises ineffective actions making it unable to learn in the LBF setting which is reflected in a consistent cumulative agent-importance score of 0.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/iql_rware-tiny-2ag-v1_agent_importance.png}
        \caption{Measurement of agent importance for IQL on RWARE}
        \label{fig:lbf_iql_imp}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/qmix_rware-tiny-2ag-v1_agent_importance.png}
        \caption{Measurement of agent importance for QMIX on RWARE}
        \label{fig:lbf_qmix_imp}
    \end{subfigure}
    \caption{Comparison of agent-importance for QMIX and IQL on the RWARE setting}
    \label{fig:iql_qmix_rware_imp}
\end{figure}

\textbf{Agent importance - limitations} The \textit{agent importance} metric although very useful is only properly applicable in certain use cases. Firstly it requires the environment to have a no-op action to be calculated correctly. Essentially to discover the agent contribution it must be able to perform an action that does nothing. In the popular SMAC setting this is not possible without directly editing the environment and must instead be approximated using a random action which creates inaccurate calculations. Additionally, most MARL settings do not have the correct features to properly calculate shapely values. Ideally for these calculations we would like to be able to reset the environment to any point in the trajectory to calculate the effect of individual agents. We instead create copies of the environment and test for all possible coalitions and while this is effective, it may not be applicable to high resource settings or cases with limited compute. This may be alleviated with the growing popularity of the JAX framework as environments designed for it's stateless computations allow states to be stored and reused in a manner similar to a resettable simulator \citep{brax2021github, gymnax2022github, jumanji2023github}.




==> sections/previous_work/5-ablation_studies.tex <==
\section{Ablation studies}

\subsection{Metric Efficiency}

\begin{table}[]
\centering
\caption{Table of the time used per metric vs the total runtime on LBF and RWARE}
\label{tab:times}
\begin{tabular}{@{}llllll@{}}
\toprule
Algorithm & Total Time & Shap & Our Shap & KL Div & Action Role \\ \midrule
IQL       & 1          & -    & 1        & 1      & 1           \\
MAPPO     & -          & 1    & 1        & 1      & 1           \\ \bottomrule
\end{tabular}
\end{table}

As these behavior explanation method require more complex calculations than using mean reward, it is reasonable to assume that calculating values like the online shapley value could affect training speed. From table \ref{tab:times} above, we can see that the metrics add minimal computational overhead even in gridworld settings aside from calculating the per step KL divergence which we recommend to calculate offline. Also as the total environment runtime increases and the environment becomes more complex, the metric runtime remains fairly consistent and is proportionally less expensive.
